Quantum association schemes

We introduce quantum association schemes. This allows to define distance regular and strongly regular quantum graphs. We bring examples thereof. In addition, we formulate the duality for translation quantum association schemes corresponding to finite quantum groups.

==> strdiag.tex <==
\usetikzlibrary{decorations.markings}
\usetikzlibrary{shapes.geometric} 
\usetikzlibrary{shapes.symbols} 
\def\Dcup{\Diagram{\draw (1,1) .. controls +(down:0.5) and +(down:0.5) .. (2,1);}}
\def\Dcap{\Diagram{\draw (1,0) .. controls +(up:0.5) and +(up:0.5) .. (2,0);}}
\def\Did{\Diagram{\draw (1,0) -- (1,1);}}
\def\Dcross{\Diagram{\draw (0,0) -- (1,1);\draw (1,0) -- (0,1);}}

\def\Rcup{\Diagram{\draw[mid arrow] (1,1) .. controls +(down:0.5) and +(down:0.5) .. (2,1);}}
\def\Lcup{\Diagram{\draw[mid arrow] (2,1) .. controls +(down:0.5) and +(down:0.5) .. (1,1);}}
\def\Rcap{\Diagram{\draw[mid arrow] (1,0) .. controls +(up:0.5) and +(up:0.5) .. (2,0);}}
\def\Lcap{\Diagram{\draw[mid arrow] (2,0) .. controls +(up:0.5) and +(up:0.5) .. (1,0);}}
\def\Fid{\Diagram{\draw[mid arrow] (1,0) -- (1,1);}}
\def\Bid{\Diagram{\draw[mid arrow] (1,1) -- (1,0);}}
\def\Fcross{\Diagram{\draw[->] (0,0) -- (1,1);\draw[->] (1,0) -- (0,1);}}

\def\textchoice#1#2#3#4#5{\ifmmode\mathchoice{#1}{#2}{#3}{#4}\else #5\fi}

\def\Diagram#1{%
\thinspace\textchoice
{\DiagramA{0.25em}{1em}{1em}{#1}}
{\DiagramA{0.25em}{0.7em}{1em}{#1}}
{\DiagramA{0.175em}{0.55em}{0.7em}{#1}}
{\DiagramA{0.125em}{0.4em}{0.5em}{#1}}
{\DiagramA{0.25em}{0.7em}{1em}{#1}}%
\thinspace%
}

\def\DiagramA#1#2#3#4{%
%\expandafter\tikzpicture\Gparam
\tikzpicture[
	%arrow styles
	mid arrow/.style={postaction={decorate,decoration={
        markings,
        mark=at position .5 with {\arrow{>}}
      }}},
	late arrow/.style={postaction={decorate,decoration={
        markings,
        mark=at position .8 with {\arrow{>}}
      }}},
	%point styles
	circ/.style={circle,draw,fill=white,inner sep=1pt},
	bcirc/.style={circle,draw,fill=black,inner sep=1pt},
	map/.style={draw,fill=white,trapezium,trapezium left angle=90,trapezium right angle=120,inner sep=1pt},
	mapC/.style={draw,fill=white,trapezium,trapezium left angle=120,trapezium right angle=90,inner sep=1pt},
	mapT/.style={draw,fill=white,trapezium,trapezium left angle=60,trapezium right angle=90,inner sep=1pt},
	mapA/.style={draw,fill=white,trapezium,trapezium left angle=90,trapezium right angle=60,inner sep=1pt},
	selfC/.style={draw,fill=white,trapezium,trapezium left angle=120,trapezium right angle=120,inner sep=1pt},
	selfCR/.style={draw,fill=white,trapezium,trapezium left angle=60,trapezium right angle=60,inner sep=1pt},
	selfT/.style={draw,fill=white,trapezium,trapezium left angle=60,trapezium right angle=120,inner sep=1pt},
	selfTR/.style={draw,fill=white,trapezium,trapezium left angle=120,trapezium right angle=60,inner sep=1pt},
	selfA/.style={draw,fill=white,signal,signal to=east,inner sep=1pt},
	selfAR/.style={draw,fill=white,signal,signal to=west,inner sep=1pt},
	square/.style={draw,fill=white,rectangle,inner sep=1pt},
	vec/.style={draw,fill=white,isosceles triangle, shape border rotate=-90,isosceles triangle apex angle=60,inner sep=1pt},
	covec/.style={draw,fill=white,isosceles triangle, shape border rotate=90,isosceles triangle apex angle=60,inner sep=1pt},
]
\pgfsetbaseline{#1}
\pgfsetxvec{\pgfpoint{#2}{0em}}
\pgfsetyvec{\pgfpoint{0em}{#3}}
\pgfsetlinewidth{\Dlinewidth em}
#4
\endtikzpicture
}

\def\Dlinewidth{0.05}

\def\DstringsB #1/#2(#3,#4){
\ifnum#1>0
\pgfmathparse{#3-(#1-1)/2}
\let\x=\pgfmathresult
\pgfmathparse{#3+(#1-1)/2}
\let\xx=\pgfmathresult
\foreach \a in {\x,...,\xx}
	\draw (\a,#4-\Dyshift) .. controls +(up:0.25) .. (#3,#4);
\fi
\ifnum#2>0
\pgfmathparse{#3-(#2-1)/2}
\let\x=\pgfmathresult
\pgfmathparse{#3+(#2-1)/2}
\let\xx=\pgfmathresult
\foreach \a in {\x,...,\xx}
	\draw (\a,#4+\Dyshift) .. controls +(down:0.25) .. (#3,#4);
\fi
}

\newcount\tmpcount
\def\Dcount#1{\ifx/#1/\else\advance\tmpcount by1\fihere\Dcount\fi}

\def\DstringsC [#1/#2](#3,#4){
\tmpcount=-1
\Dcount#1//
\pgfmathparse{#3-\the\tmpcount/2}
\let\x=\pgfmathresult
\scope[
	up arrow/.style={postaction={decorate,decoration={
        markings,
        mark=at position .3 with {\arrow{>}}
      }}},
	down arrow/.style={postaction={decorate,decoration={
        markings,
        mark=at position .3 with {\arrow{<}}
      }}},
]
\DstringsD{#3}{#4}#1//
\endscope
\tmpcount=-1
\Dcount#2//
\pgfmathparse{#3-\the\tmpcount/2}
\let\x=\pgfmathresult
\scope[
	down arrow/.style={postaction={decorate,decoration={
        markings,
        mark=at position .7 with {\arrow{>}}
      }}},
	up arrow/.style={postaction={decorate,decoration={
        markings,
        mark=at position .7 with {\arrow{<}}
      }}},
]
\DstringsE{#3}{#4}#2//
\endscope
}

\def\fihere#1\fi{\fi#1}
\def\DstringsD#1#2#3{\ifx/#3/\else
	\csname D#3\endcsname (\x,#2-\Dyshift) .. controls +(up:0.25) .. (#1,#2);
	\pgfmathparse{\x+1}
	\let\x=\pgfmathresult
	\fihere\DstringsD{#1}{#2}\fi
}
\def\DstringsE#1#2#3{\ifx/#3/\else
	\csname D#3\endcsname (\x,#2+\Dyshift) .. controls +(down:0.25) .. (#1,#2);
	\pgfmathparse{\x+1}
	\let\x=\pgfmathresult
	\fihere\DstringsE{#1}{#2}\fi
}

\def\Dstrings{
\futurelet\nextchar\DstringsA
}

\def\DstringsA{\ifx[\nextchar\let\next=\DstringsC\else\let\next=\DstringsB\fi\next}

\def\Dmor#1#2 (#3,#4){
\def\Dyshift{0.5}
\ifx;#2;\else\Dstrings#2(#3,#4)\fi
\node at (#3,#4) [#1] {};
}

\def\DMor#1#2 (#3,#4)#5{
\def\Dyshift{1}
\ifx;#2;\else\Dstrings#2(#3,#4)\fi
\node at (#3,#4) [#1] {#5};
}

\def\spider{\futurelet\nextchar\spiderA}
\def\spiderA{\ifx[\nextchar\def\next[##1]{\Diagram{\Dmor{bcirc}[##1] (1,0.5)}}\else\def\next##1{\Diagram{\Dmor{bcirc}##1 (1,0.5)}}\fi\next}
\def\wspider{\futurelet\nextchar\wspiderA}
\def\wspiderA{\ifx[\nextchar\def\next[##1]{\Diagram{\Dmor{circ}[##1] (1,0.5)}}\else\def\next##1{\Diagram{\Dmor{circ}##1 (1,0.5)}}\fi\next}

\def\Ddef#1#2{\expandafter\def\csname D#1\endcsname{#2}}
\Ddef>{\draw[<-]}
\Ddef<{\draw[>-]}
\Ddef-{\draw}
\Ddef={\draw[very thick]}
\expandafter\def\csname D0\endcsname#1;{}
\expandafter\def\csname D.\endcsname (#1,#2)#3;{\node at (#1,#2) {$\dots$};}

\endinput

